PHANTOM: Curating GitHub for engineered software projects using time-series clustering

Context: Within the field of Mining Software Repositories, there are numerous methods employed to filter datasets in order to avoid analysing low-quality projects. Unfortunately, the existing filtering methods have not kept up with the growth of existing data sources, such as GitHub, and researchers often rely on quick and dirty techniques to curate datasets. Objective: The objective of this study is to develop a method capable of filtering large quantities of software projects in a resource-efficient way. Method: This study follows the Design Science Research (DSR) methodology. The proposed method, PHANTOM, extracts five measures from Git logs. Each measure is transformed into a time-series, which is represented as a feature vector for clustering using the k-means algorithm. Results: Using the ground truth from a previous study, PHANTOM was shown to be able to rediscover the ground truth on the training dataset, and was able to identify "engineered" projects with up to 0.87 Precision and 0.94 Recall on the validation dataset. PHANTOM downloaded and processed the metadata of 1,786,601 GitHub repositories in 21.5 days using a single personal computer, which is over 33% faster than the previous study which used a computer cluster of 200 nodes. The possibility of applying the method outside of the open-source community was investigated by curating 100 repositories owned by two companies. Conclusions: It is possible to use an unsupervised approach to identify engineered projects. PHANTOM was shown to be competitive compared to the existing supervised approaches while reducing the hardware requirements by two orders of magnitude.

==> features.tex <==

\newcommand{\lenCategory}{1.8cm}
\newcommand{\lenDescription}{7cm}
\begin{table}
    \centering
    \caption[PHANTOM Features]{Features extracted by PHANTOM}
    \label{tab:features}
    \begin{tabular}{p{\lenCategory} | l p{\lenDescription}}
        \hline\noalign{\smallskip}
    
    Duration                    & Duration & Time interval in weeks between the first and last week of the time-series\\
    \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{8}{\lenCategory}{Y value}    & Max y & The highest value\\
                                & Max y Pos & The week number of the Max Y\\
                                & Mean y & The average value\\
                                & Sum y & The sum of all values\\
                                & q25 & The 25\% quantile of values\\
                                & q50 & The 50\% quantile of values\\
                                & q75 & The 75\% quantile of values\\
                                & std & The standard deviation of values\\
    \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{3}{\lenCategory}{Peaks}        & Peak down & The number of downwards facing peaks\\
                                & Peak none & The number of peaks that are neither downwards, nor upwards facing peaks\\
                                & Peak up   & The number of upwards facing peaks\\
    \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{3}{\lenCategory}{Time between peaks} & Min TBP up & \multirow{3}{\lenDescription}{The time between upwards facing peaks is measured as the number of weeks between two neighbouring peaks.}\\
                                        & Avg TBP up & \\
                                        & Max TBP up & \\
    \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{3}{\lenCategory}{Amplitude}     & Min amplitude & \multirow{3}{\lenDescription}{The amplitude is the difference in height between a peak and the previous valley. This value is normalised by dividing it with Max Y.}\\
                                & Avg amplitude & \\
                                & Max amplitude & \\
                                
    \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{6}{\lenCategory}{Positive and negative peak deviation}     & Min PPD & \multirow{3}{\lenDescription}{The positive peak deviation (PPD) is the difference between the Mean Y value and the y value of a upwards facing peak.}\\
                                                            & Avg PPD & \\
                                                            & Max PPD & \\
                                                            & Min NPD & \multirow{3}{\lenDescription}{The negative peak deviation (NPD) is the difference between the Mean Y value the y value of a downwards facing peak.}\\
                                                            & Avg NPD & \\
                                                            & Max NPD & \\
                                                            
    \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{6}{\lenCategory}{Positive and negative sequences}& Min PS & \multirow{6}{\lenDescription}{A sequence is, when at least two sequential gradients have the same sign. Therefore, the positive (PS) and negative sequences (NS) are numeric values, that count the number of sequential same sign gradients.}\\
                                                    & Avg PS & \\
                                                    & Max PS & \\
                                                    & Min NS & \\
                                                    & Avg NS & \\
                                                    & Max NS & \\
                                                    
    \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{8}{\lenCategory}{Positive and negative gradients}& Min PG & \multirow{6}{\lenDescription}{Gradients are the difference between two neighbouring y values.}\\
                                                    & Avg PG & \\
                                                    & Max PG & \\
                                                    & Min NG & \\
                                                    & Avg NG & \\
                                                    & Max NG & \\ \noalign{\smallskip}\cline{2-3}\noalign{\smallskip}
                                                    & PG Count & Number of positive gradients (PG)\\
                                                    & NG Count & Number of negative gradients (NG)\\
    \noalign{\smallskip}\hline
    \end{tabular}
\end{table}

==> old-parts.tex <==
\subsection{The method Performs Well On Commodity Hardware At Large-Scale (Req5)}
\label{sec:validation_R5}

PHANTOM was used to download the Organisation, Utility, Negative Instances and Validation datasets. In order to validate that PHANTOM is applicable at scale, the timings of PHANTOM are extrapolated to the size of the large dataset. Since the Organisation dataset comes from a different selection process than the other datasets, it is not used for this extrapolation. 

PHANTOM's results (see Table \ref{table:timings}) show that 3.8\% of the repositories were unavailable, which means they have been deleted or made private. The total download time was 7.5 minutes for 500 repositories, which gives the average repository-download time of 0.94 seconds. 

When these values are extrapolated up to the Large dataset (1,857,423 repositories), the time to obtain the Git logs is estimated to be 20.2 days. This extrapolation validates that PHANTOM can perform well on commodity hardware, even at large scale. 


\begin{table}
    \centering
        \caption[PHANTOM Timings]{Number of available repositories and timings to clone and generate the Git log for them.}
    \label{table:timings}
    \begin{tabular}{l|cc}
    \hline\noalign{\smallskip}
    Dataset & Available Repositories & Time Taken (minutes)  \\ 
    \noalign{\smallskip}\hline\noalign{\smallskip}
    Organisation                    & 149 / 150              & 10:39    \\
    Utility                         & 145 / 150              & 2:44        \\
    Negative Instances              & 138 / 150              & 1:53        \\
    Validation(Well-engineered)     & 100 / 100              & 1:36        \\
    Validation(Not well-engineered) & 98 / 100               & 1:18        \\
    \noalign{\smallskip}\hline
    \end{tabular}%

\end{table}


\section{Old abstract}

\textcolor{red}{TODO: update the abstract - remember that: ``Please provide an abstract of 150 to 250 words. The abstract should not contain any undefined abbreviations or unspecified references''}
\noindent Context: Within the field of Mining Software Repositories, there are numerous methods employed to filter datasets in order to avoid analysing low-quality projects, such as backups and student projects. Since the rise of GitHub, the world’s largest repository hosting site, large scale analysis has become more common. However, filtering methods have not kept up with this growth and researchers often rely on quick and dirty techniques to curate datasets. 

\noindent Objective: The objective of this study is to develop a method that clusters large quantities of software projects in a limited time frame. This explores the possibility that a fully-automated method can be used to identify high-quality repositories at large scale and in the absence of an established ground-truth. At the same time, the hardware requirements and time limitations of existing approaches should be reduced to remove the barrier for researchers.

\noindent Method: This study follows the Design Science Research methodology. The proposed method, PHANTOM, extracts five measures from Git logs. Each measure is transformed into a time-series, which is represented as a feature vector for clustering using a k-means algorithm. 

\noindent Results: Using the ground-truth from a previous study, PHANTOM was shown to be competitive compared to supervised approaches while reducing the hardware requirements by two orders of magnitude. The ground-truth was rediscovered by several k-means models, with some models achieving up to 0.87 Precision or 0.94 Recall. The highest Matthews correlation coefficient (MCC) was 0.65. The method was later applied to over 1.77 million repositories obtained from GitHub and found that 38\% of them are ``well-engineered''. The method also shows that cloning repositories is a viable alternative to the GitHub API and GHTorrent when collecting metadata.

\noindent Conclusions: It is possible to use an unsupervised approach to identify projects of high-quality. PHANTOM's reference implementation, called PHANTOM, downloaded and processed the metadata of 1,786,601 GitHub repositories in 21.5 days, which is over 33\% faster than a similar study, which used a computer cluster of 200 nodes. PHANTOM is flexible and can be improved further, but it already shows excellent results. The method is able to filter repositories very accurately with low hardware requirements and was able to rediscover an established ground-truth.

% validation

By applying PHANTOM to classify repositories in the labeled datasets, we could directly compare its accuracy to the \emph{reaper}'s. However, we decided to extend the validation by comparing the results provided by both methods for the Large dataset. Unfortunately, in this case the analysis is speculative since there is no ground-truth established for the dataset. Nevertheless, it could show how similar or different the results could be when both methods are used to classify unseen cases in the real-life context.
